On Approximate Nearest Neighbour Selection for Multi-Stage Dense Retrieval

Dense retrieval, which describes the use of contextualised language models such as BERT to identify documents from a collection by leveraging approximate nearest neighbour (ANN) techniques, has been increasing in popularity. Two families of approaches have emerged, depending on whether documents and queries are represented by single or multiple embeddings. ColBERT, the exemplar of the latter, uses an ANN index and approximate scores to identify a set of candidate documents for each query embedding, which are then re-ranked using accurate document representations. In this manner, a large number of documents can be retrieved for each query, hindering the efficiency of the approach. In this work, we investigate the use of ANN scores for ranking the candidate documents, in order to decrease the number of candidate documents being fully scored. Experiments conducted on the MSMARCO passage ranking corpus demonstrate that, by cutting of the candidate set by using the approximate scores to only 200 documents, we can still obtain an effective ranking without statistically significant differences in effectiveness, and resulting in a 2x speedup in efficiency.

==> approximation.tex <==
\section{Background \& Related Work}

\section{Large-Scale Nearest Neighbour Search}

Given $N$ real-valued data vectors with $D$ dimensions $\{x_1, \ldots, x_N\}$ and a query vector $q$, nearest neighbour (NN) search aims at finding the closest data vector to the query vector, according to some distance. The naive solution relies on a linear scan of the data vectors, and can be implemented exploiting vectorised operations on modern CPUs/GPus, as well as high-performance matrix computation libraries such as BLAS. For large values of $N$, this approach requires too much time, hence approximate NN (ANN) search is standard alternative. ANN does not necessarily compute the exact neighbours, but it trades off accuracy with runtime speed and memory consumption.

For million-scale data sets, many ANN tehcniques exists, such as locality-sensitive hashing, mapping similar items to the same symbol with high probability~\citemissing, kd-tree forests, recursively partitioning the input items along the dimension of maximum variance~\citemissing, and (hierarchical) navigable small world graphs, storing the items into vertices and neighbour relationships into edges~\citemissing. These methods have a large memory consumption, that can be reduced by product quantization (PQ) strategies~\citemissing.

In PQ, every data vector is split into $M \ll D$ sub-vectors, generating $M$ sets of $N$ vectors with $\lceil D/M \rceil$ dimensions. The items in each of these set are quantised independently from the other set through k-means into $K$ representative vectors (centroids). Hence, an input item $x \in \mathbb{R}^D$ is represented by the quantised item $\bar{x} \in \{1, \ldots, K\}^M$. The distance between a query vector $q$ and an input vector $x$ can be approximated by computing the distance the query and the quantised input vector $\bar{x}$.

In order to deal with billion-scale data sets, inverted files are used in conjunction with product quantisation (IVFPQ). Firsly, the input space is partitioned into $L$ sub-spaces by a coarse quantiser based on k-means. Every input item $x$ is assigned to the sub-space with the closest centroid $c$ and ``centered'', i.e., represented in that sub-space by its residual $r = x - c$. All residuals in the same sub-space are quantised with PQ, and stored into a posting list of $(i, bar{r}_i)$ pairs, sorted w.r.t. the distance from the corresponding centroid. In order to perform ANN search over IVFPQ, the input query is mapped into the closest among the $L$ sub-spaces with the coarse quantiser, its residual computed, and then the closest element in the sub-space is identified by PQ approximated distance computations.
When looking for the top $k$ closest elements instead of the single closest one, one sup-space could not contain all $k$ elements, due to the coarse quantisation. Hence, instead of looking into the closest sub-space only, a few more sub-space, in increasing order of distance, are probed, and their approximate distance used to select the top $k$ closest elements across all probed sub-spaces.

\inote{at the end, I'm not sure how much of this section we need}

==> h3.tex <==

Finally, we note that Hypotheses H1 \& H2 implicitly address Limitation 3 by aiming to identify the most useful embeddings among all of the query embeddings. However, in doing so, they assume query term independence -- that we can identify the best query terms without comparing to the other query terms. This is akin to the probabilistic ranking principle applied to query terms; instead we argue that an effective subset of the query embeddings would not include masked tokens that are nearly identical to the original query tokens, nor those of other masked tokens. \nic{To this end, we pose the following hypothesis:}

\begin{hyp}[H\ref{hyp:diverse}] \label{hyp:diverse}
An effective ordering of query embeddings will promote terms that are both important and different from the other query embeddings.
\end{hyp}

To address this hypothesis, we are inspired by document ranking approaches that go beyond the classical probabilistic ranking principle, such as those addressing diversity in document retrieval~\cite{divFNT2015}. In particular, we adapt the classical Maximal Marginal Relevance (MMR) approach~\cite{carbonell1998use} in order to identify \nic{those query} embeddings that are both important and diverse. In particular, MMR is formulated as a \nic{query embeddings} re-ranking process, \inote{not to be confused with our document re-ranking at second stage} where, at each iteration, among an initial set of query embeddings $R(q) = \{\phi_1, \ldots, \phi_{|q|}\}$, the next embedding to be selected into the final set $\mathcal{P}(q)$ is one that is both important, and sufficiently distinct from those embeddings already selected in $\mathcal{P}(q)$:
\begin{equation}\label{eq:mmr}
    \argmax_{\phi_i \in R(q)} \Big[ \alpha \cdot s(\phi_i) - (1-\alpha) \cdot \max_{\phi_j \in \mathcal{P}(q)} d(\phi_i,\phi_j) \Big]
\end{equation}
% $$
% MRR = \argmax_{qt \in R} \big[ \lambda \cdot P(qt|q) -  (1-\lambda) \cdot \max_{qt' \in S} Sim(qt'|qt) \big]
% $$
In this formulation, the free parameter $0 \leq \alpha \leq 1$ controls the balance between importance and diversity; \nic{the function $d(\phi_i, \phi_j)$ measure the similarity between a given query embeddings $\phi_i$ and previously selected query embedding $\phi_j$. To measure this similarity, we use the cosine similarity.}
